ATA: Adaptive Task Allocation for Efficient Resource Management in Distributed Machine Learning

Asynchronous methods are fundamental for parallelizing computations in distributed machine learning. They aim to accelerate training by fully utilizing all available resources. However, their greedy approach can lead to inefficiencies using more computation than required, especially when computation times vary across devices. If the computation times were known in advance, training could be fast and resource-efficient by assigning more tasks to faster workers. The challenge lies in achieving this optimal allocation without prior knowledge of the computation time distributions. In this paper, we propose ATA (Adaptive Task Allocation), a method that adapts to heterogeneous and random distributions of worker computation times. Through rigorous theoretical analysis, we show that ATA identifies the optimal task allocation and performs comparably to methods with prior knowledge of computation times. Experimental results further demonstrate that ATA is resource-efficient, significantly reducing costs compared to the greedy approach, which can be arbitrarily expensive depending on the number of workers.

==> Sections/todos.tex <==
\section{Francesco's remarks}


\textbf{TO DO: how the regret is connected to the actual objectives in federated learning? If not connected, minimizing regret would be unjustified. Maybe the regret is actually not what we want, instead we should directly say we want a result like the one in \Cref{cor:main} --- section 2}

\textbf{TO DO: Add something here explaining why this problem is hard: non-convexity, partial feedback, online, etc. --- section 2}

\textbf{TO DO: first, tell me what are the shortcomings of ATA. Then, tell me the proposed solution and its advantages both from a theoretical point of view (bound) and from a practical point of view (less exploration on useless arms?). Finally, tell me the trade-off in terms of what I need to know. --- section 4}

\textbf{TO DO: maybe better here to state the result, or at least to be more explicit on what are the differences with the result for ATA. --- section 4 }

\textbf{TO DO: add new lemma on empirical concentration to make theory people happy. --- 6.2}

\textbf{TO DO: this could go after intro or after algorithm. Depending on the position, the discussion can be more or less detailed. --- sections 3.1 and 4}

\textbf{TO DO: add proof sketch -- Section 5.1}

